Airway Mucus Rheology: Physical Insights for Navigating through Health to Pathology and Clinical Applications

Airway mucus is a complex gel with an anisotropic three-dimensional network structure. As a crucial component of the respiratory defense barrier, it plays a vital role in maintaining airway hydration and supporting the function of airway epithelial cells. Through linear and nonlinear rheological mechanisms such as ciliary motion and coughing, airway mucus expels foreign pathogens and toxic nano- and microparticles while selectively allowing the passage of specific nutrients and proteins. These protective and clearance functions depend on the proper rheological properties of mucus under normal physiological conditions. However, in respiratory disease such as CF, COPD, asthma, and COVID-19, excessive mucus secretion is often accompanied by abnormal rheological behaviors. This leads to impaired mucus flow, airway obstruction, and potentially life-threatening conditions. Therefore, this review examines the rheological behaviors of airway mucus in relation to health and disease, focusing on both macrorheology and microrheology. The review highlights those changes in the chemical composition and microstructure of airway mucus, especially under pathological conditions, that can significantly alter its rheological behavior. Rheological parameters can also serve as biological indicators to study the role of mucus in clearance functions and aid in developing pulmonary drug delivery systems. By integrating findings from both macro- and microrheological studies, this review aims to enhance our understanding of the complex behavior of airway mucus, supporting better diagnosis, treatment, and management of chronic respiratory diseases.

==> Pic.tex <==
\begin{figure}[tbph]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/Active microrheology.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

\begin{table}[htp!]
\centering
\begin{tabular}{|l|p{12cm}|}
\hline
